Hyper-Reduced Autoencoders for Efficient and Accurate Nonlinear Model Reductions

Projection-based model order reduction on nonlinear manifolds has been recently proposed for problems with slowly decaying Kolmogorov n-width such as advection-dominated ones. These methods often use neural networks for manifold learning and showcase improved accuracy over traditional linear subspace-reduced order models. A disadvantage of the previously proposed methods is the potential high computational costs of training the networks on high-fidelity solution snapshots. In this work, we propose and analyze a novel method that overcomes this disadvantage by training a neural network only on subsampled versions of the high-fidelity solution snapshots. This method coupled with collocation-based hyper-reduction and Gappy-POD allows for efficient and accurate surrogate models. We demonstrate the validity of our approach on a 2d Burgers problem.

==> references.tex <==
@article{choi,
  title={A fast and accurate physics-informed neural network reduced order model with shallow masked autoencoder},
  author={Kim, Youngkyu and Choi, Youngsoo and Widemann, David and Zohdi, Tarek},
  journal={arXiv preprint arXiv:2009.11990},
  year={2020}
}

@article{ryckelynck2005priori,
  title={A priori hyperreduction method: an adaptive approach},
  author={Ryckelynck, David},
  journal={Journal of computational physics},
  volume={202},
  number={1},
  pages={346--366},
  year={2005},
  publisher={Elsevier}
}

@article{farhat2014dimensional,
  title={Dimensional reduction of nonlinear finite element dynamic models with finite rotations and energy-based mesh sampling and weighting for computational efficiency},
  author={Farhat, Charbel and Avery, Philip and Chapman, Todd and Cortial, Julien},
  journal={International Journal for Numerical Methods in Engineering},
  volume={98},
  number={9},
  pages={625--662},
  year={2014},
  publisher={Wiley Online Library}
}

@article{bishop1995training,
  title={Training with noise is equivalent to Tikhonov regularization},
  author={Bishop, Chris M},
  journal={Neural computation},
  volume={7},
  number={1},
  pages={108--116},
  year={1995},
  publisher={MIT Press}
}

@inproceedings{dhifallah2021inherent,
  title={On the inherent regularization effects of noise injection during training},
  author={Dhifallah, Oussama and Lu, Yue},
  booktitle={International Conference on Machine Learning},
  pages={2665--2675},
  year={2021},
  organization={PMLR}
}

@article{poole2014analyzing,
  title={Analyzing noise in autoencoders and deep networks},
  author={Poole, Ben and Sohl-Dickstein, Jascha and Ganguli, Surya},
  journal={arXiv preprint arXiv:1406.1831},
  year={2014}
}

@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013}
}

@software{Falcon_PyTorch_Lightning_2019,
author = {Falcon, William and {The PyTorch Lightning team}},
doi = {10.5281/zenodo.3828935},
license = {Apache-2.0},
month = {3},
title = {{PyTorch Lightning}},
url = {https://github.com/Lightning-AI/lightning},
version = {1.4},
year = {2019}
}
@article{rizzi2020pressio,
  title={Pressio: Enabling projection-based model reduction for large-scale nonlinear dynamical systems},
  author={Rizzi, Francesco and Blonigan, Patrick J and Parish, Eric J and Carlberg, Kevin T},
  journal={arXiv preprint arXiv:2003.07798},
  year={2020}
}

@article{romor2022non,
  title={Non-linear manifold ROM with Convolutional Autoencoders and Reduced Over-Collocation method},
  author={Romor, Francesco and Stabile, Giovanni and Rozza, Gianluigi},
  journal={arXiv preprint arXiv:2203.00360},
  year={2022}
}

@article{lee2020model,
  title={Model reduction of dynamical systems on nonlinear manifolds using deep convolutional autoencoders},
  author={Lee, Kookjin and Carlberg, Kevin T},
  journal={Journal of Computational Physics},
  volume={404},
  pages={108973},
  year={2020},
  publisher={Elsevier}
}

@article{tencer2021tailored,
  title={A tailored convolutional neural network for nonlinear manifold learning of computational physics data using unstructured spatial discretizations},
  author={Tencer, John and Potter, Kevin},
  journal={SIAM Journal on Scientific Computing},
  volume={43},
  number={4},
  pages={A2581--A2613},
  year={2021},
  publisher={SIAM}
}

@book{goodfellow2016deep,
  title={Deep learning},
  author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron},
  year={2016},
  publisher={MIT press}
}

@article{everson1995karhunen,
  title={Karhunen--Loeve procedure for gappy data},
  author={Everson, Richard and Sirovich, Lawrence},
  journal={JOSA A},
  volume={12},
  number={8},
  pages={1657--1664},
  year={1995},
  publisher={Optical Society of America}
}

@article{willcox2006unsteady,
  title={Unsteady flow sensing and estimation via the gappy proper orthogonal decomposition},
  author={Willcox, Karen},
  journal={Computers \& fluids},
  volume={35},
  number={2},
  pages={208--226},
  year={2006},
  publisher={Elsevier}
}

@book{brunton2019data,
  title={Data-driven science and engineering: Machine learning, dynamical systems, and control},
  author={Brunton, Steven L and Kutz, J Nathan},
  year={2019},
  publisher={Cambridge University Press}
}

@article{loshchilov2017decoupled,
  title={Decoupled weight decay regularization},
  author={Loshchilov, Ilya and Hutter, Frank},
  journal={arXiv preprint arXiv:1711.05101},
  year={2017}
}

@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@article{paszke2019pytorch,
  title={Pytorch: An imperative style, high-performance deep learning library},
  author={Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and others},
  journal={Advances in neural information processing systems},
  volume={32},
  pages={8026--8037},
  year={2019}
}

@article{lauzon2022s,
  title={S-OPT: A points selection algorithm for hyper-reduction in reduced order models},
  author={Lauzon, Jessica T and Cheung, Siu Wun and Shin, Yeonjong and Choi, Youngsoo and Copeland, Dylan Matthew and Huynh, Kevin},
  journal={arXiv preprint arXiv:2203.16494},
  year={2022}
}

@misc{enwiki:1037710578,
    author = "{Wikipedia contributors}",
    title = "Project Jupyter --- {Wikipedia}{,} The Free Encyclopedia",
    year = "2021",
    url = "https://en.wikipedia.org/w/index.php?title=Project_Jupyter&oldid=1037710578",
    note = "[Online; accessed 20-August-2021]"
  }
  
  @book{holmes2012turbulence,
  title={Turbulence, coherent structures, dynamical systems and symmetry},
  author={Holmes, Philip and Lumley, John L and Berkooz, Gahl and Rowley, Clarence W},
  year={2012},
  publisher={Cambridge university press}
}

@article{choi2020sns,
  title={SNS: A solution-based nonlinear subspace method for time-dependent model order reduction},
  author={Choi, Youngsoo and Coombs, Deshawn and Anderson, Robert},
  journal={SIAM Journal on Scientific Computing},
  volume={42},
  number={2},
  pages={A1116--A1146},
  year={2020},
  publisher={SIAM}
}

@article{berry2005algorithm,
  title={Algorithm 844: Computing sparse reduced-rank approximations to sparse matrices},
  author={Berry, Michael W and Pulatova, Shakhina A and Stewart, GW},
  journal={ACM Transactions on Mathematical Software (TOMS)},
  volume={31},
  number={2},
  pages={252--269},
  year={2005},
  publisher={ACM New York, NY, USA}
}

@article{carlberg2013gnat,
  title={The GNAT method for nonlinear model reduction: effective implementation and application to computational fluid dynamics and turbulent flows},
  author={Carlberg, Kevin and Farhat, Charbel and Cortial, Julien and Amsallem, David},
  journal={Journal of Computational Physics},
  volume={242},
  pages={623--647},
  year={2013},
  publisher={Elsevier}
}


